A Discontinuous Galerkin Fast Spectral Method for the Full Boltzmann Equation with General Collision Kernels

The Boltzmann equation, an integro-differential equation for the molecular distribution function in the physical and velocity phase space, governs the fluid flow behavior at a wide range of physical conditions, including compressible, turbulent, as well as flows involving further physics such as non-equilibrium internal energy exchange and chemical reactions. Despite its wide applicability, deterministic solution of the Boltzmann equation presents a huge computational challenge, and often the collision operator is simplified for practical reasons. In this work, we introduce a highly accurate deterministic method for the full Boltzmann equation which couples the Runge-Kutta discontinuous Galerkin (RKDG) discretization in time and physical space (Su et al., Comp. Fluids, 109 pp. 123-136, 2015) and the recently developed fast Fourier spectral method in velocity space (Gamba et al., SIAM J. Sci. Comput., 39 pp.~B658--B674, 2017). The novelty of this approach encompasses three aspects: first, the fast spectral method for the collision operator applies to general collision kernels with little or no practical limitations, and in order to adapt to the spatial discretization, we propose here a singular-value-decomposition based algorithm to further reduce the cost in evaluating the collision term; second, the DG formulation employed has high order of accuracy at element-level, and has shown to be more efficient than the finite volume method; thirdly, the element-local compact nature of DG as well as our collision algorithm is amenable to effective parallelization on massively parallel architectures. The solver has been verified against analytical Bobylev-Krook-Wu solution. Further, the standard benchmark test cases of rarefied Fourier heat transfer, Couette flow, oscillatory Couette flow, normal shock wave, lid-driven cavity flow, and thermally driven cavity flow have been studied.

==> plots/dummy.tex <==
\begin{tikzpicture}[scale=1.0]

	\draw[dashed] (0,0) -- (6,0) -- (6,4) -- (0,4) -- (0,0);		% big rectangle
	
\end{tikzpicture}

==> plots/journalPaper-jfmSchematic.tex <==
\begin{tikzpicture}[scale=1]
	\def\W{6};
	\def\H{4};
	\def\pW{0.15};	% pattern width
	\def\aW{1};
	\def\aH{0.75};

	\draw (0,0) -- (\W,0) -- (\W,\H) -- (0,\H) -- (0,0);		% big rectangle
	
	\draw[thick, line width=0.6mm] (0,0) -- (0,\H);
	\draw[thick, line width=0.6mm] (\W,0) -- (\W,\H);
	
	\fill[pattern=north west lines, pattern color=gray, line width = 0.1mm, thin] (0,0) rectangle ({-\pW},\H);
	\fill[pattern=north east lines, pattern color=gray, line width = 0.1mm, thin] (\W,0) rectangle ({\W+\pW},\H);
	
	\draw[thick,-latex, line width=0.40mm] ({\W*0.75},{\H*0.5}) -- ({\W*0.75+\aW},{\H*0.5});	% left arrow
	\draw[thick,-latex, line width=0.40mm] ({\W*0.25},{\H*0.5}) -- ({\W*0.25-\aW},{\H*0.5});	% left arrow
	\node[] at ({\W*0.5},{\H*0.5}) {Walls};					% freestream

	\draw[domain=0:23mm, samples=100, black, xshift={\W*0.6 cm}, yshift={\H cm}, -latex, thick] plot ({-2*cos(\x)},{-sin(\x)}) node[anchor=west] {Periodic};
	
	\draw[domain=0:23mm, samples=100, black, xshift={\W*0.6 cm}, yshift={0 cm}, -latex, thick] plot ({-2*cos(\x)},{sin(\x)}) node[anchor=west] {Periodic};
	
		
	\draw[thick,-latex, line width=0.45mm, black] (0,0) -- (0,1);				% x-axis
	\draw[thick,-latex, line width=0.45mm, black] (0,0) -- (1,0);				% y-axis
	
	\node[] at (0.5,-0.4) {$x$};
	\node[] at (-0.4,0.4) {$y$};
\end{tikzpicture}

==> plots/journalPaper-jfmSchematic1D.tex <==
%\begin{tikzpicture}
%		\draw[decorate sep={1mm}{4mm}, fill](0,0) -- (4,0) ;
%		\draw(0,0) -- (4,0) ;
%		\draw[blue] (0.0,0.0) circle (0.1cm);
%		\draw[red] (4.0,0.0) circle (0.1cm);
%		
%		\draw[-latex] (0.0,-0.5) -- (0.0, 0.0) node[below, yshift=-0.5cm] {$T_l=263K$};
%		\draw[-latex] (4.0,-0.5) -- (4.0, 0.0) node[below, yshift=-0.5cm] {$T_r=283K$};
%		
%		\draw[-latex] (-2.0,-1) -- (-1.0, -1) node[anchor=north] {x};
%		\draw[-latex] (-2.0,-1) -- (-2.0, 0) node[anchor=south] {y};
%\end{tikzpicture}

\begin{tikzpicture}
		%\draw[decorate sep={1mm}{4mm}, fill](0,0) -- (4,0) ;
		\def\pr{1.23};
		\foreach \x in {1,...,5}
			\fill ({-\pr + (\pr)^\x},0cm) circle (0.05cm);
			
		\foreach \x in {1,...,5}
				\fill ({ 4 + \pr - (\pr)^(\x)},0cm) circle (0.05cm);

		\draw(0,0) -- (4,0) ;
		\draw[blue] (0.0,0.0) circle (0.1cm);
		\draw[red] (4.0,0.0) circle (0.1cm);
		
		\draw[-latex] (0.0,-0.5) -- (0.0, 0.0) node[below, yshift=-0.5cm] {$\mathbf{u}_l,\;T_l$};
		\draw[-latex] (4.0,-0.5) -- (4.0, 0.0) node[below, yshift=-0.5cm] {$\mathbf{u}_r,\;T_r$};
		
		\draw[-latex] (-2.0,-1) -- (-1.0, -1) node[anchor=north] {x};
		\draw[-latex] (-2.0,-1) -- (-2.0, 0) node[anchor=south] {y};
\end{tikzpicture}

==> plots/lidCavitySchematic.tex <==
\begin{tikzpicture}[scale=0.9]		
	\def\W{5};
	\def\H{5};
	\def\pW{0.15};	% pattern width
	\def\aW{0.75};
	\def\aH{0.75};
	
	\draw (0,0) -- (\W,0) -- (\W,\H) -- (0,\H) -- (0,0);		% big rectangle
		
	%\draw[thick, line width=0.6mm] (0,0) -- (0,\H);
	%\draw[thick, line width=0.6mm] (\W,0) -- (\W,\H);
		
	\fill[pattern=north west lines, pattern color=gray, line width = 0.1mm, thin] (0,0) rectangle ({-\pW},\H);
	\fill[pattern=north east lines, pattern color=gray, line width = 0.1mm, thin] (\W,0) rectangle ({\W+\pW},\H);
		
	\fill[pattern=north west lines, pattern color=gray, line width = 0.1mm, thin] (0,0) rectangle (\W,{-\pW});
	\fill[pattern=north east lines, pattern color=gray, line width = 0.1mm, thin] (0,\H) rectangle ({\W},{\H+\pW});
		
	\draw[thick,-latex, line width=0.40mm] ({\W*0.75},{\H*0.5}) -- ({\W*0.75+\aW},{\H*0.5});	% left arrow
	\draw[thick,-latex, line width=0.40mm] ({\W*0.25},{\H*0.5}) -- ({\W*0.25-\aW},{\H*0.5});	% right arrow
	\draw[thick,-latex, line width=0.40mm] ({\W*0.5},{\H*0.5-\aH}) -- ({\W*0.5},{\aH});	% bottom arrow
	\node[] at ({\W*0.5},{\H*0.5}) {Fixed Walls};					% freestream
	
	%\draw[domain=0:23mm, samples=100, black, xshift={\W*0.6 cm}, yshift={\H cm}, -latex, thick] plot ({-2*cos(\x)},{-sin(\x)}) node[anchor=west] {$T_f$};
	\node[] at ({\W*0.5},{\H*0.75}) {Moving Wall};					% freestream
	\draw[thick,-latex, line width=0.40mm] ({\W*0.5},{\H*0.85}) -- ({\W*0.5},{\H*1.1-\aH});	% top arrow
	\draw[thick,-latex, line width=0.40mm] ({\aW},{\H+\aH}) -- ({\W-\aW},{\H+\aH}) node[anchor=south east] {$u$};	% moving wall
	
	%\draw[domain=0:23mm, samples=100, black, xshift={\W*0.6 cm}, yshift={0 cm}, -latex, thick] plot ({-2*cos(\x)},{sin(\x)}) node[anchor=west] {$T_f$};
				
	\draw[thick,-latex, line width=0.45mm, black] (0,0) -- (0,1);				% x-axis
	\draw[thick,-latex, line width=0.45mm, black] (0,0) -- (1,0);				% y-axis
		
	\node[] at (0.5,-0.4) {$x$};
	\node[] at (-0.4,0.4) {$y$};	
\end{tikzpicture}

==> plots/polyhedralMeshSchematic3d.tex <==
\usetikzlibrary{calc}

\newcommand*\rows{5}

\begin{tikzpicture}[scale=1.3]
	%top-left
	\def\colu {gray};
	
	%\draw[step=1cm,gray,very thin] (-1.9,-1.9) grid (5.9,5.9);
	
		%\pgfmathsetmacro{\cj}{\rows-\k};
		%\foreach \row in {2, ...,\rows} {
		%\foreach \col in {\row, ..., \rows} {
		%	\draw (\col, \row) -- ({\col+1}, \row);
		%	\draw (\col, \row) -- (\col, {\row+1});
		%	\draw (\col, \row) -- ({\col+1}, {\row+1});
		%}
		%}
		
		%\foreach \i in {2,3,..., \rows} 
		%{
		%	\pgfmathsetmacro{\cj}{\rows-\i};
		%	\pgfmathsetmacro{\ck}{2*\i-1};
		%	\pgfmathsetmacro{\one}{1};
		%	\pgfmathsetmacro{\two}{1};
			
		%	\foreach \k in {1,2,..., \ck} 
		%	{
					
		%		\ifx\k\ck
		%		\else								
		%			\draw ({\cj+\k-1}, {\i}) -- ({\cj+\k+1}, {\i});
		%		\fi
				
					%\draw ({\cj+\k}, {\i}) -- ({\cj+\k+1}, {\i-1});
				
				%\ifx\i\rows
				%\else
				%	\draw ({\cj+\k}, {\i}) -- ({\cj+\k}, {\i+1});
				%\fi
			%}
		%}
					
							
		
	\begin{scope}
	    \clip(0,0.9) rectangle (5,4);
	\foreach \row in {0,1, 2, ...,\rows} 
	{
	    \draw ($\row*(0.5, {0.5*sqrt(3)})$) -- ($(\rows,0)+\row*(-0.5, {0.5*sqrt(3)})$);
	    \draw ($\row*(1, 0)$) -- ($(\rows/2,{\rows/2*sqrt(3)})+\row*(0.5,{-0.5*sqrt(3)})$);
	    \draw ($\row*(1, 0)$) -- ($(0,0)+\row*(0.5,{0.5*sqrt(3)})$);
	}
	\end{scope}   
	\node at (2.5,2.05) {$p$};
	\fill (2.5,2.58) circle (0.05cm);
	\fill (2.00,1.72) circle (0.05cm);
	\fill (3.00,1.72) circle (0.05cm);
	\fill (2.25,2.14) circle (0.05cm);
	\fill (2.75,2.14) circle (0.05cm);
	\fill (2.5,1.73) circle (0.05cm);
	
	\fill (3.85,3.55) circle (0.05cm);
	\node at (4.5,3.5) {$N(p)$};
	
	%\draw[\colu] (0,0) -- (-2,1.5) -- (0,4) -- (2,2) -- (0,0);		% front
	
	%\draw[\colu] (0,0) -- (0,-2);
	%\draw[\colu] (0,-2) -- (2.2,-0.5);
	%\draw[\colu] (2.2,-0.5) -- (2,2);
	
	%\draw[\colu] (0,4) -- (-0.3,1);
	%\draw[\colu,dashed] (-0.3,1) -- (2.2, -0.5);
	
	%\draw[\colu] (-0.3,1) -- (-2.2,-1.0);
	%\draw[\colu] (-2.2,-1.0) -- (0, -2);
	%\draw[\colu] (-2.2,-1.0) -- (-2, 1.5);
	
	% top-pentagon
	%\draw[\colu] (0,4) -- (-2.5,4.5);
	%\draw[\colu] (-2.5,4.5) -- (-5.5,3.5);
	%\draw[\colu] (-5.5,3.5) -- (-4.5,1.7);
	%\draw[\colu] (-4.5,1.7) -- (-2,1.5);
	
	% bottom-pentagon
	%\draw[\colu, dashed] (-0.3,1) -- (-2.5,2);
	%\draw[\colu, dashed] (-2.5,2) -- (-6.5,1.0);
	%\draw[\colu] (-6.5,1) -- (-5.5,-1.2);
	%\draw[\colu] (-5.5,-1.2) -- (-2.2,-1.0);
	
	% join top-bottom pentagon
	%\draw[\colu] (-6.5,1.0) -- (-5.5,3.5);
	%\draw[\colu] (-5.5,-1.2) -- (-4.5,1.7);
	%\draw[\colu, dashed] (-2.5,4.5) -- (-2.5,2);
	
	% face
	%\fill[gray, fill opacity=0.1] (0,4) -- (-0.3,1) -- (-2.2,-1) -- (-2,1.5) node[yshift=0.8cm, xshift=1.1cm, black, fill opacity=1] {$f$};
	
	% point p
	%\fill[gray] (-2.65,1.90) circle (0.15cm) node[yshift=-0.5cm, xshift=-0.15cm, black] {$p$}; 
	
	% point n
	%\fill[gray] (0,0.5) circle (0.15cm) node[yshift=-0.5cm, xshift=0.25cm, black] {$N$}; 
	
	% join p to n
	%\draw[-latex, line width=0.02cm] (-2.65,1.90) -- (0,0.5);
	
	% face vector
	%\draw[-latex, line width=0.02cm] (-1,1.5) -- (0.7,1.0) node[yshift=0.3cm, xshift=0cm, black] {$s_f$};
	
\end{tikzpicture}

==> plots/thermalCavitySchematic.tex <==
\begin{tikzpicture}[scale=0.9]		
		\def\W{6};
		\def\H{4};
		\def\pW{0.15};	% pattern width
		\def\aW{1};
		\def\aH{0.75};
	
		\draw (0,0) -- (\W,0) -- (\W,\H) -- (0,\H) -- (0,0);		% big rectangle
		
		%\draw[thick, line width=0.6mm] (0,0) -- (0,\H);
		%\draw[thick, line width=0.6mm] (\W,0) -- (\W,\H);
		
		\fill[pattern=north west lines, pattern color=gray, line width = 0.1mm, thin] (0,0) rectangle ({-\pW},\H);
		\fill[pattern=north east lines, pattern color=gray, line width = 0.1mm, thin] (\W,0) rectangle ({\W+\pW},\H);
		
		\fill[pattern=north west lines, pattern color=gray, line width = 0.1mm, thin] (0,0) rectangle (\W,{-\pW});
		\fill[pattern=north east lines, pattern color=gray, line width = 0.1mm, thin] (0,\H) rectangle ({\W},{\H+\pW});
		
		\draw[thick,-latex, line width=0.40mm] ({\W*0.75},{\H*0.5}) -- ({\W*0.75+\aW},{\H*0.5});	% left arrow
		\draw[thick,-latex, line width=0.40mm] ({\W*0.25},{\H*0.5}) -- ({\W*0.25-\aW},{\H*0.5});	% left arrow
		\node[] at ({\W*0.5},{\H*0.5}) {$T_c$};					% freestream
	
		\draw[domain=0:23mm, samples=100, black, xshift={\W*0.6 cm}, yshift={\H cm}, -latex, thick] plot ({-2*cos(\x)},{-sin(\x)}) node[anchor=west] {$T_f$};
		
		\draw[domain=0:23mm, samples=100, black, xshift={\W*0.6 cm}, yshift={0 cm}, -latex, thick] plot ({-2*cos(\x)},{sin(\x)}) node[anchor=west] {$T_f$};
		
			
		\draw[thick,-latex, line width=0.45mm, black] (0,0) -- (0,1);				% x-axis
		\draw[thick,-latex, line width=0.45mm, black] (0,0) -- (1,0);				% y-axis
		
		\node[] at (0.5,-0.4) {$x$};
		\node[] at (-0.4,0.4) {$y$};	


		% Draw mesh
		\def\pr{1.22};
		\foreach \y in {1,...,5}
			\foreach \x in {1,...,9} {
				\draw[dotted] ({-\pr + (\pr)^\x},{-\pr + (\pr)^\y}) -- ({-\pr + (\pr)^(\x+1)},{-\pr + (\pr)^(\y)});
			}

		\foreach \y in {1,...,5}
			\foreach \x in {1,...,9} {
				\draw[dotted] ({-\pr + (\pr)^\x},{4 + \pr - (\pr)^\y}) -- ({-\pr + (\pr)^(\x+1)},{4 + \pr - (\pr)^(\y)});
			}

		\foreach \y in {1,...,5}
			\foreach \x in {1,...,6} {
				\draw[dotted] ({-\pr + (\pr)^\x},{-\pr + (\pr)^\y}) -- ({-\pr + (\pr)^(\x)},{-\pr + (\pr)^(\y+1)});
			}

		\foreach \y in {1,...,5}
			\foreach \x in {1,...,6} {
				\draw[dotted] ({-\pr + (\pr)^\x},{4 + \pr - (\pr)^\y}) -- ({-\pr + (\pr)^(\x)},{4 + \pr - (\pr)^(\y+1)});
			}

		\foreach \y in {1,...,5}
			\foreach \x in {1,...,6} {
				\draw[dotted] ({6 + \pr - (\pr)^\x},{-\pr + (\pr)^\y}) -- ({6 + \pr - (\pr)^(\x)},{-\pr + (\pr)^(\y+1)});
			}

		\foreach \y in {1,...,5}
			\foreach \x in {1,...,6} {
				\draw[dotted] ({6 + \pr - (\pr)^\x},{4 + \pr - (\pr)^\y}) -- ({6 + \pr - (\pr)^(\x)},{4 + \pr - (\pr)^(\y+1)});
			}
			
		%\foreach \x in {1,...,5}
		%		\fill ({ 4 + \pr - (\pr)^(\x)},0cm) circle (0.05cm);

		
		\def\Off{0.75};
		
		\draw[dashed](0,-\Off) -- (0,-{\H+\Off});
		\draw[dashed] (0,-{\H+\Off}) node[anchor=east] {$T_c$} -- (\W,-{\H+\Off}) node[anchor=north east] {\footnotesize Temperature profile : $T_f$};
		\draw[dashed](\W,-\Off) -- (\W,-{\H+\Off});
		\draw(0,-{\H+\Off}) -- (\W/2,-\Off);
		\draw (\W/2,-\Off) -- (\W,-{\H+\Off});		
		\draw[dotted] (0,-\Off) node[anchor=east] {$T_h$} -- (\W/2,-\Off);
	\end{tikzpicture}
